Large Language Model Distilling Medication Recommendation Model

The recommendation of medication is a vital aspect of intelligent healthcare systems, as it involves prescribing the most suitable drugs based on a patient's specific health needs. Unfortunately, many sophisticated models currently in use tend to overlook the nuanced semantics of medical data, while only relying heavily on identities. Furthermore, these models face significant challenges in handling cases involving patients who are visiting the hospital for the first time, as they lack prior prescription histories to draw upon. To tackle these issues, we harness the powerful semantic comprehension and input-agnostic characteristics of Large Language Models (LLMs). Our research aims to transform existing medication recommendation methodologies using LLMs. In this paper, we introduce a novel approach called Large Language Model Distilling Medication Recommendation (LEADER). We begin by creating appropriate prompt templates that enable LLMs to suggest medications effectively. However, the straightforward integration of LLMs into recommender systems leads to an out-of-corpus issue specific to drugs. We handle it by adapting the LLMs with a novel output layer and a refined tuning loss function. Although LLM-based models exhibit remarkable capabilities, they are plagued by high computational costs during inference, which is impractical for the healthcare sector. To mitigate this, we have developed a feature-level knowledge distillation technique, which transfers the LLM's proficiency to a more compact model. Extensive experiments conducted on two real-world datasets, MIMIC-III and MIMIC-IV, demonstrate that our proposed model not only delivers effective results but also is efficient. To ease the reproducibility of our experiments, we release the implementation code online.

==> 4Experiment_backup.tex <==
\section{Experiment}

In this section, we will analyze the proposed LEADER by comprehensive experiments on two real-world datasets. We explore the following Research Questions (\textbf{RQ}) to illustrate the findings:

\begin{itemize}[leftmargin=*]
    \item \textbf{RQ1}: How the proposed LEADER perform compared with current state-of-the-art medication recommendation models?
    \item \textbf{RQ2}: Do all designs for LEADER take effect?
    \item \textbf{RQ3}: How do the designed knowledge distillation and profile alignment affect the performance of LEADER?
    \item \textbf{RQ4}: Can the proposed student model conduct medication recommendation with a high efficiency?
\end{itemize}

\subsection{Experimental Settings}

\subsubsection{\textbf{Dataset}}

    The datasets used in the experiments are from Medical Information Mart for Intensive Care (MIMIC)~\footnote{https://mimic.mit.edu/}. There are two versions available currently, \ie MIMIC-III and MIMIC-IV. MIMIC-III collects data from 2001 to 2012, while MIMIC-IV contains records from 2008 to 2019. For the preprocessing, we transform the NDC code of the medications to ATC level codes to get the drug-drug interaction (DDI) graph and molecule connection graph for the implementation of the baselines. Besides, we only retain the prescriptions during the first 24 hours of a visit, as previous works~\cite{shang2019gamenet,yang2021safedrug} did. We filter out the medications that cannot be mapped to ATC codes and the visits that have void input set. At last, we split the data into train/validation/test by the ratio of 8:1:1. The statistics of the preprocessed data are shown in Table~\ref{tab:exp_dataset}.

%% 单栏表
%%% Statistics of Datasets %%%
\begin{table}[]
\centering
\caption{The statistics of the preprocessed datasets}
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{c|cc}
\toprule[1pt]
\textbf{Item} & \textbf{MIMIC-III} & \textbf{MIMIC-IV} \\ \midrule
\# of single-visit patients & 908 & 2,877 \\
\# of multi-visit patients & 5,442 & 6,029 \\
diag. / proc. / med. space size & 1,958 / 1,430 / 112 & 1,998 / 1,001 / 125 \\
avg. / max of diag. per visit & 10.51 / 128 & 8.41 / 220 \\
avg. / max of proc. per visit & 3.84 / 50 & 2.11 / 49 \\
avg. / max of med. per visit & 11.64 / 64 & 7.02 / 72 \\ 
\bottomrule[1pt]
\end{tabular}
}
\label{tab:exp_dataset}
\vspace{-4mm}
\end{table}
%%% Statistics of Datasets %%%

\subsubsection{\textbf{Baselines}}
    In the experiments, we compare our LEADER with several state-of-the-art medication recommendation models:
    \begin{itemize}[leftmargin=*]
        \item \textbf{RETAIN}~\cite{choi2016retain}. RETAIN designs a two-level attention model to enhance the accuracy and interpretability of clinical variable prediction. We implement it by adding the representation of diagnosis and procedure for each visit.
        \item \textbf{G-Bert}~\cite{shang2019pre}. G-Bert utilizes all the data to pre-train diagnosis and medication encoders, but needs historical medication records in fine-tuning stage.
        \item \textbf{GAMENet}~\cite{shang2019gamenet}. GAMENet adopts the memory bank to integrate global medication interaction and drug-drug interaction knowledge. For the implementation, we substitute the retrieval representation from patient history with the one from patient similarity for those single-visit patients.
        \item \textbf{SafeDrug}~\cite{yang2021safedrug}. SafeDrug utilizes drug molecule structure to encode the medications and add direct drug-drug interaction control during the training process. 
        \item \textbf{MICRON}~\cite{yang2021change}. MICRON finds that there is little distinction between the prescription in two successive visits and thus captures the change for the final recommendation. For the input, the medication set taken on the last visit is compulsory.
        \item \textbf{COGNet}~\cite{wu2022conditional}. COGNet copies the ever-prescribed drugs to the current visit, so the previous medication records are necessary.
        \item \textbf{REFINE}~\cite{bhoi2023refine}. REFINE proposes to model the severity of the drug-drug interaction and the fine-grained medication dosage. For a fair comparison, we implement it by inputting the diagnosis rather than lab test responses to the model. Since REFINE also takes the historical medication records as input, it cannot infer for single-visit patients.
    \end{itemize}
    
    \noindent To verify the ability of the LLM for medication recommendation, we compare the modified LLM proposed in Section~\ref{sec:method_LLM}, which is denoted as \textbf{LEADER(T)}. Also, the distilled student model is marked as \textbf{LEADER(S)} in the following experiments.


%%% Overall Experiments on MIMIC-III %%%
\begin{table*}[]
\centering
\tabcolsep=0.05cm   % 调整列间距
\caption{The overall results of competing baselines and LEADER on MIMIC-III. The boldface refers to the highest score and the underline indicates the best result of the models. ``\textbf{{\Large *}}'' indicates the statistically significant improvements (\ie two-sided t-test with $p<0.05$) over the best baseline. ``-'' represents the model cannot acquire the corresponding results due to the inability to the single-visit patients.}
\label{tab:exp_mimic3}
\resizebox{1\textwidth}{!}{
% \fontsize{6pt}{8.5pt}\selectfont
\centering
\begin{tabular}{c|ccc|ccc|ccc}
\toprule[1pt]
\multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c|}{\textbf{Overall}} & \multicolumn{3}{c|}{\textbf{Multi-visit}} & \multicolumn{3}{c}{\textbf{Single-visit}} \\ \cmidrule{2-10} 
 & \textbf{PRAUC} & \textbf{Jaccard} & \textbf{F1} & \textbf{PRAUC} & \textbf{Jaccard} & \textbf{F1} & \textbf{PRAUC} & \textbf{Jaccard} & \textbf{F1} \\ \midrule
RETAIN & 0.7513 $\pm$ 0.0025 & 0.4943 $\pm$ 0.0023 & 0.6516 $\pm$ 0.0022 & 0.7580 $\pm$ 0.0020 & 0.5106 $\pm$ 0.0023 & 0.6674 $\pm$ 0.0022 & 0.7337 $\pm$ 0.0067 & 0.4811 $\pm$ 0.0053 & 0.6403 $\pm$ 0.0049 \\
G-Bert & - & - & - & 0.6904 $\pm$ 0.0017 & 0.4578 $\pm$ 0.0019 & 0.6186 $\pm$ 0.0018 & - & - & - \\
GAMENet & 0.7605 $\pm$ 0.0011 & 0.5024 $\pm$ 0.0010 & 0.6595 $\pm$ 0.0008 & 0.7638 $\pm$ 0.0023 & 0.5070 $\pm$ 0.0028 & 0.6635 $\pm$ 0.0025 & 0.7451 $\pm$ 0.0053 & 0.4840 $\pm$ 0.0038 & 0.6442 $\pm$ 0.0036 \\
SafeDrug & 0.7582 $\pm$ 0.0020 & 0.5054 $\pm$ 0.0024 & 0.6621 $\pm$ 0.0021 & 0.7623 $\pm$ 0.0029 & 0.5095 $\pm$ 0.0027 & 0.6658 $\pm$ 0.0024 & 0.7416 $\pm$ 0.0044 & 0.4900 $\pm$ 0.0043 & 0.6481 $\pm$ 0.0042 \\
MICRON & - & - & - & 0.7651 $\pm$ 0.0027 & 0.5110 $\pm$ 0.0025 & 0.6741 $\pm$ 0.0023 & - & - & - \\
COGNet & - & - & - & 0.7771 $\pm$ 0.0019 & \underline{0.5275 $\pm$ 0.0021} & \underline{0.6805 $\pm$ 0.0019} & - & - & - \\
REFINE & - & - & - & 0.7791 $\pm$ 0.0017 & 0.5235 $\pm$ 0.0018 & 0.6794 $\pm$ 0.0017 & - & - & - \\ \midrule
\textbf{LEADER(T)} & \textbf{0.7816 $\pm$ 0.0015}* & \textbf{0.5391 $\pm$ 0.0015}* & \textbf{0.6921 $\pm$ 0.0014}* & \textbf{0.7854 $\pm$ 0.0015}* & \textbf{0.5450 $\pm$ 0.0021}* & \textbf{0.6971 $\pm$ 0.0018}* & \underline{0.7590 $\pm$ 0.0046}* & \textbf{0.5090 $\pm$ 0.0044}* & \textbf{0.6668 $\pm$ 0.0041}* \\ 
\textbf{LEADER(S)} & \underline{0.7795 $\pm$ 0.0025}* & \underline{0.5175 $\pm$ 0.0022}* & \underline{0.6737 $\pm$ 0.0019}* & \underline{0.7830 $\pm$ 0.0019} & 0.5208 $\pm$ 0.0020 & 0.6768 $\pm$ 0.0017 & \textbf{0.7631 $\pm$ 0.0056}* & \underline{0.5038 $\pm$ 0.0062}* & \underline{0.6614 $\pm$ 0.0057}* \\ 
\bottomrule[1pt]
\end{tabular}
}
\vspace{-2mm}
\end{table*}
%%% Overall Experiments on MIMIC-III %%%


\subsubsection{\textbf{Implementation Details}}

    All experiments in this paper are conducted on the Intel Xeon Gold 6133 platform with Tesla V100 32G GPUs. The code is based on Python 3.6.5 and PyTorch 1.12.0. As for the LLM-based medication recommendation, \ie LEADER(T), we adopt the LlaMA-7B~\footnote{https://github.com/facebookresearch/llama/tree/llama\_v1}~\cite{touvron2023llama} as the foundation model in this paper. During the fine-tuning, the LoRA layers are accompanied by the layers identified as ``q\_proj'', ``k\_proj'', ``v\_proj'', ``o\_proj'', ``down\_proj'', ``up\_proj'' and ``gate\_proj'' in LLM. Other configurations include LoRA rank of $8$, batch size of $32$, learning rate of $2e-4$ and maximum input length of $2,048$. Due to different data scales, the maximum training steps are set to 3,000 and 4,000 for MIMIC-III and MIMIC-IV, respectively. In terms of the distillation for the student model LEADER(S), we set the dimension $d_e$ and $d_t$ to $64$, the number of transformer layers of all encoders $\mathcal{E}$ to $1$ and $\tau$ to $1$. We adopt Adam optimizer~\cite{kingma2014adam} and set the learning rate to $5e-4$. The batch size is fixed at $4$ for MIMIC-III and $16$ for MIMIC-IV. The best hyper-parameters are chosen by the PRAUC metric on the validation set. Specifically, $\alpha$ is tuned from $0.1$ to $0.9$, while $\beta$ is searched from $\{0.1, 0.05, 0.01, 0.005, 0.001\}$. To facilitate the reproduction of our model, we release the code online~\footnote{https://github.com/liuqidong07/LEADER-pytorch}.


\subsubsection{\textbf{Evaluation Metrics}}

    Following the previous works~\cite{shang2019gamenet,yang2021safedrug,wu2022conditional,bhoi2023refine}, we apply three common metrics to evaluate the proposed model, \ie \textit{Precision-Recall AUC} (\textbf{PRAUC} $\uparrow$), \textit{Jaccard Similarity Score} (\textbf{Jaccard} $\uparrow$) and \textit{Average F1 Score} (\textbf{F1} $\uparrow$). To guarantee the robustness of the experimental results, we adopt bootstrapping sampling during the test process. In detail, we randomly sample $80\%$ samples in each round and the metrics shown below are the averaged on $10$-round tests.


%%% Overall Experiments on MIMIC-IV %%%
\begin{table*}[]
\centering
\tabcolsep=0.05cm   % 调整列间距
\caption{The overall results of competing baselines and LEADER on MIMIC-IV. The boldface refers to the highest score and the underline indicates the best result of the models. ``\textbf{{\Large *}}'' indicates the statistically significant improvements (\ie two-sided t-test with $p<0.05$) over the best baseline. ``-'' represents the model cannot acquire the corresponding results due to the inability to the single-visit patients.}
\label{tab:exp_mimic4}
\resizebox{1\textwidth}{!}{
\begin{tabular}{c|ccc|ccc|ccc}
\toprule[1pt]
\multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c|}{\textbf{Overall}} & \multicolumn{3}{c|}{\textbf{Multi-visit}} & \multicolumn{3}{c}{\textbf{Single-visit}} \\ \cmidrule{2-10} 
 & \textbf{PRAUC} & \textbf{Jaccard} & \textbf{F1} & \textbf{PRAUC} & \textbf{Jaccard} & \textbf{F1} & \textbf{PRAUC} & \textbf{Jaccard} & \textbf{F1} \\ \midrule
RETAIN & 0.6574 $\pm$ 0.0055 & 0.4152 $\pm$ 0.0044 & 0.5688 $\pm$ 0.0043 & 0.6576 $\pm$ 0.0044 & 0.4161 $\pm$ 0.0038 & 0.5693 $\pm$ 0.0040 & 0.6588 $\pm$ 0.0055 & 0.4165 $\pm$ 0.0035 & 0.5707 $\pm$ 0.0042 \\
G-Bert & - & - & - & 0.6237 $\pm$ 0.0028 & 0.3727 $\pm$ 0.0021 & 0.5169 $\pm$ 0.0022 & - & - & - \\
GAMENet & 0.6720 $\pm$ 0.0030 & 0.4336 $\pm$ 0.0032 & 0.5871 $\pm$ 0.0030 & 0.6731 $\pm$ 0.0030 & 0.4339 $\pm$ 0.0020 & 0.5877 $\pm$ 0.0021 & 0.6671 $\pm$ 0.0049 & 0.4292 $\pm$ 0.0041 & 0.5819 $\pm$ 0.0040 \\
SafeDrug & 0.6706 $\pm$ 0.0025 & 0.4295 $\pm$ 0.0027 & 0.5820 $\pm$ 0.0024 & 0.6752 $\pm$ 0.0031 & 0.4331 $\pm$ 0.0018 & 0.5860 $\pm$ 0.0017 & 0.6641 $\pm$ 0.0072 & 0.4214 $\pm$ 0.0073 & 0.5749 $\pm$ 0.0073 \\
MICRON & - & - & - & 0.6660 $\pm$ 0.0041 & 0.4414 $\pm$ 0.0027 & 0.5951 $\pm$ 0.0027 & - & - & - \\
COGNet & - & - & - & 0.6873 $\pm$ 0.0034 & \underline{0.4638 $\pm$ 0.0028} & \underline{0.6119 $\pm$ 0.0026} & - & - & - \\
REFINE & - & - & - & 0.6977 $\pm$ 0.0042 & 0.4538 $\pm$ 0.0047 & 0.6063 $\pm$ 0.0044 & - & - & - \\ \midrule
\textbf{LEADER(T)} & \textbf{0.7120 $\pm$ 0.0024}* & \textbf{0.4779 $\pm$ 0.0021}* & \textbf{0.6296 $\pm$ 0.0020}* & \textbf{0.7238 $\pm$ 0.0031}* & \textbf{0.4895 $\pm$ 0.0033}* & \textbf{0.6400 $\pm$ 0.0032}* & \underline{0.6881 $\pm$ 0.0039}* & \textbf{0.4539 $\pm$ 0.0026}* & \textbf{0.6071 $\pm$ 0.0026}* \\ 
\textbf{LEADER(S)} & \underline{0.7020 $\pm$ 0.0022}* & \underline{0.4483 $\pm$ 0.0025}* & \underline{0.6005 $\pm$ 0.0026}* & \underline{0.6994 $\pm$ 0.0037} & 0.4500 $\pm$ 0.0031 & 0.6023 $\pm$ 0.0029 & \textbf{0.7033 $\pm$ 0.0041}* & \underline{0.4420 $\pm$ 0.0039}* & \underline{0.5946 $\pm$ 0.0039}* \\ 
\bottomrule[1pt]
\end{tabular}
}
% \vspace{-4mm}
\end{table*}
%%% Overall Experiments on MIMIC-IV %%%


\subsection{Overall Performance (RQ1)}

    To respond to the research question (\textbf{RQ1}), we reveal the performance comparison between the proposed method and competitors in Table~\ref{tab:exp_mimic3} and Table~\ref{tab:exp_mimic4}. Then, we address the analysis of the results.

    Overall, LEADER(T) performs a strong lead compared with all of the other models on two datasets, which indicates the semantic understanding ability of the LLM. At the same time, the distilled student model, marked as LEADER(S), also outperforms existing state-of-the-art medication recommendation models. This phenomenon shows the success of the designed distillation enhancement. 

    Then, we probe the performance comparison according to different patient groups. As mentioned before, some recent baselines, \eg G-Bert, MICRON, COGNet and REFINE, consider the historical medication records as one of the necessary inputs, so they do not have the results for single-visit patients. We first observe the multi-visit patient group. G-Bert performs the worst, because it does not take patient's procedures into consideration. Then, we can find that the three baselines (MICRON, COGNet and REFINE), which model the historical prescriptions explicitly, can outperform the other competitors in the multi-visit group. Such comparison illustrates utilizing previous drug records can actually benefit the recommendation for the current visit. The proposed LEADER(T) can surpass all models consistently due to the powerful ability of the LLM. As for the designed LEADER(S), it can outperform others on the PRAUC metric, but is worse than COGNet on Jaccard and F1. We think the reason lies in that COGNet adopts beam search to generate the final recommendations, but it faces efficiency issues.

    In terms of the performance in single-visit and overall groups, GAMENet and SafeDrug are better than RETAIN, because they model the relations between medications more carefully by EHR graph and molecule graph. However, they still underperform the two variants of the proposed LEADER consistently. On the one hand, LEADER can utilize the historical information and surpass baselines in the multi-visit group largely, which contributes to the overall scores. On the other hand, due to the semantic understanding ability of LLMs, LEADER(T) and LEADER(S) both surpass competitors in the single-visit group on two datasets. It is worth noting that the distilled LEADER(S) is even better than LEADER(T) in the single-visit group under the PRAUC metric. This phenomenon indicates the benefits of the combination of collaborative signals from the student model and semantic information from LLMs. 

    From the analysis, we conclude that the proposed LLM-based medication recommendation model shows a greater \textbf{semantic understanding ability} and \textbf{single-visit ability} than conventional models. Besides, the designed distillation method can actually enhance the derived student model.

%%% Ablation Study %%%
\begin{table*}[]
\centering
\caption{The ablation study on two datasets. Due to limited space, only PRAUC scores are shown in the table.}
\label{tab:exp_ablation}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{c|ccc|ccc}
\toprule[1pt]
\multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c|}{\textbf{MIMIC-III}} & \multicolumn{3}{c}{\textbf{MIMIC-IV}}  \\ \cmidrule{2-7} 
 & \textbf{Overall} & \textbf{Multi-visit} & \textbf{Single-visit} & \textbf{Overall} & \textbf{Multi-visit} & \textbf{Single-visit} \\ \midrule
\textbf{LEADER(S)} & 0.7795 $\pm$ 0.0025 & 0.7830 $\pm$ 0.0019 & 0.7631 $\pm$ 0.0056 & 0.7020 $\pm$ 0.0022 & 0.6994 $\pm$ 0.0037 & 0.7033 $\pm$ 0.0041 \\ \midrule
\textit{w/o} KD & 0.7673 $\pm$ 0.0026 & 0.7720 $\pm$ 0.0034 & 0.7464 $\pm$ 0.0052 & 0.6840 $\pm$ 0.0031 & 0.6853 $\pm$ 0.0044 & 0.6768 $\pm$ 0.0062 \\
\textit{w/o} feature-KD & 0.7672 $\pm$ 0.0024 & 0.7730 $\pm$ 0.0034 & 0.7448 $\pm$ 0.0058 & 0.6846 $\pm$ 0.0023 & 0.6865 $\pm$ 0.0028 & 0.6792 $\pm$ 0.0047 \\
\textit{w/o} align & 0.7774 $\pm$ 0.0017 & 0.7836 $\pm$ 0.0031 & 0.7579 $\pm$ 0.0054 & 0.6967 $\pm$ 0.0026 & 0.6987 $\pm$ 0.0039 & 0.6939 $\pm$ 0.0026  \\
\textit{w/o} shared $\mathcal{E}_{Visit}$ & 0.7781 $\pm$ 0.0010 & 0.7830 $\pm$ 0.0022 & 0.7613 $\pm$ 0.0050 & 0.6985 $\pm$ 0.0021 & 0.7001 $\pm$ 0.0035 & 0.6923 $\pm$ 0.0045  \\
\bottomrule[1pt]
\end{tabular}
}
% \vspace{-4mm}
\end{table*}
%%% Ablation Study %%%

\subsection{Ablation Study (RQ2)}

    To verify the effectiveness of each proposed component for LEADER, we conduct ablation experiments. The results are shown in Table~\ref{tab:exp_ablation}. Firstly, we aim to validate how the designed feature-level knowledge distillation has an effect on the student model. \textit{w/o KD} represents we remove the KD loss directly during the training of LEADER(S), while \textit{w/o feature-KD} denotes using the KL-divergence of output probability between student and teacher model as the KD loss~\cite{hinton2015distilling}. From the results, we can find that these two variants both underperform the proposed LEADER(S) by a large margin. The drastic performance drop indicates that the feature-level knowledge distillation can actually enhance the collaborative student model. Also, the designed feature-level KD is more suitable for knowledge transfer from LLMs than traditional output-level KD.

    Then, we seek to explore whether our design for the student model is reasonable. In Table~\ref{tab:exp_ablation}, \textit{w/o align} means that we leave out the profile alignment module proposed in Section~\ref{sec:method_align}. The experimental results illustrate that the alignment benefits the single-visit group more, which contributes to the overall performance elevation. The reason may be that the alignment can refine the representation of the profile, which is considered the only medication record for single-visit patients. \textit{w/o shared $\mathcal{E}_{Visit}$} represents that the designed student model adopts a split visit encoder for diagnosis, procedure and medication. This variant is worse than LEADER(S), which shows that the shared encoder can help learn more general medical knowledge. As the response to \textbf{RQ2}, we can conclude that the designed feature-level KD and other components in the student model are all beneficial to LEADER(S).



%%%% Hyper-parameter Experiments %%%%%
\begin{figure}[t]
\centering
\includegraphics[width=1\linewidth]{figures/Exp_KD.pdf}
%\vspace{-5mm}
\caption{The results of experiments for the weight of knowledge distillation loss $\alpha$ on two datasets.}
\label{fig:exp_KD}
% \vspace{-2mm}
\end{figure}
%%%% Hyper-parameter Experiments %%%%%

%%%% Hyper-parameter Experiments %%%%%
\begin{figure}[t]
\centering
\includegraphics[width=1\linewidth]{figures/Exp_CL.pdf}
%\vspace{-5mm}
\caption{The results of experiments for the weight of alignment loss $\beta$ on two datasets.}
\label{fig:exp_CL}
% \vspace{-5mm}
\end{figure}
%%%%% Hyper-parameter Experiments %%%%%

\subsection{Hyper-parameter Analysis (RQ3)}

    To answer the \textbf{RQ3}, we adjust the strength of knowledge distillation and profile alignment during the training. The Figure~\ref{fig:exp_KD} and Figure~\ref{fig:exp_CL} show the performance change according to $\alpha$ and $\beta$, respectively. We observe that the performance of LEADER(S) rises when $\alpha$ increases in a certain range. This phenomenon indicates that the knowledge transfer from the LLM-based teacher model can benefit the collaborative model. However, too large scale of KD loss will confuse the model training towards the ground-truth labels, so the PRAUC score drops with the continual increase of $\alpha$. The best values of $\alpha$ for MIMIC-III and MIMIC-IV are $0.4$ and $0.8$, respectively. In terms of profile alignment, the figure shows the general performance trend is up at first and then down with $\beta$ change from $0.1$ to $0$. The reason why PRAUC increases at first is that too large strength of contrastive loss will be harmful to the model convergence. In contrast, since the alignment can help refine the representation of the profile, the PRAUC drops when $\beta$ then decreases to $0$. As a result, the best $\beta$ for MIMIC-III and MIMIC-IV are $5e^{-3}$ and $1e^{-2}$, respectively.


\subsection{Efficiency Analysis (RQ4)}

% \begin{table}[!t]
% \centering
% \caption{The performance and inference cost comparison between LLMs and distilled small model. The performance is evaluated by Jaccard and F1 score. The inference cost is measured by averaged inference time per sample and necessary GPU memory.}
% \label{tab:exp_efficiency}
% \resizebox{0.47\textwidth}{!}{
% \begin{tabular}{ccccc}
% \toprule[1pt]
% \multicolumn{5}{c}{\textbf{MIMIC-III}} \\ \midrule
% \multicolumn{1}{c|}{\textbf{Model}} & \textbf{Jaccard} & \multicolumn{1}{c|}{\textbf{F1}} & \textbf{Latency} & \textbf{Memory} \\ \midrule
% \multicolumn{1}{c|}{LLM} & 0.4395 & \multicolumn{1}{c|}{0.6023} & 4.4850 s & 17,017 MB \\
% \multicolumn{1}{c|}{LEADER(T)} & 0.5391 & \multicolumn{1}{c|}{0.6921} & 0.4535 s & 17,319 MB \\
% \multicolumn{1}{c|}{LEADER(S)} & 0.5170 & \multicolumn{1}{c|}{0.6732} & 0.0181 s & 1,209 MB \\ 
% \midrule[1pt]
% \multicolumn{5}{c}{\textbf{MIMIC-IV}} \\ 
% \midrule
% \multicolumn{1}{c|}{\textbf{Model}} & \textbf{Jaccard} & \multicolumn{1}{c|}{\textbf{F1}} & \textbf{Latency} & \textbf{Memory} \\ \midrule
% \multicolumn{1}{c|}{LLM} & 0.4190 & \multicolumn{1}{c|}{0.5732} & 4.3274 s & 17,017 MB \\
% \multicolumn{1}{c|}{LEADER(T)} & 0.4779 & \multicolumn{1}{c|}{0.6296} & 0.5561 s & 17,735 MB \\
% \multicolumn{1}{c|}{LEADER(S)} & 0.4483 & \multicolumn{1}{c|}{0.6005} & 0.0186 s & 1,211 MB \\ 
% \bottomrule[1pt]
% \end{tabular}
% }
% \vspace{-6mm}
% \end{table}

%%%%% Efficiency Figure %%%%%
\begin{figure}[t]
\centering
\includegraphics[width=1\linewidth]{figures/Exp_efficiency.pdf}
%\vspace{-5mm}
\caption{The performance and inference cost comparison between LLMs and distilled small model. The performance is evaluated by (a) Jaccard and (b) F1 score. The inference cost is measured by (c) averaged inference time per sample and (d) necessary GPU memory.}
\label{fig:exp_efficiency}
\vspace{-4mm}
\end{figure}
%%%%% Efficiency Figure %%%%%

    As mentioned before, inference efficiency is an important issue in medical applications. Thus, we compare the efficiency between the LLM-based model and collaborative student model to respond \textbf{RQ4}. We apply the latency and GPU memory to measure the efficiency. In detail, the latency is calculated by averaging the total inference time of the test set on the number of test samples. Thus, the latency represents the average waiting time to complete the recommendation for one patient. The memory is the minimum GPU memory requirement for inference. The performance and efficiency comparisons are shown in Figure~\ref{fig:exp_efficiency}. In the figure, \textit{LLM} denotes the general LLM, which outputs the medication name as the final recommendation. It is worth noting that, for a fair comparison, we adopt the same fine-tuning method (\ie LoRA) and foundation model (\ie LlaMA-7b) for \textit{LLM} and LRADER(T) in the experiments.

    Observing the performance comparison, \textit{LLM} underperforms the LLM-based LEADER(T) with a large gap and is even worse than LEADER(S). The results illustrate that the general LLM for recommendation faces the \textbf{out-of-corpus} challenge introduced in Section~\ref{sec:intro}. In contrast, our modified LLM can better inspire the semantic understanding ability of LLM to complete the medication recommendation task. As for the efficiency comparison, we can find that LEADER(T) has a shorter latency than general \textit{LLM}. It is caused by the beam search during the word token generation, while the modified LLM can give out the probability in one run. In a word, the proposed modification of LLM can elevate effectiveness and efficiency simultaneously. However, both LLM-based medication recommendation models still pose the \textbf{high inference costs} problem. From the results, the proposed LEADER(S) can implement $25 \times \sim 30 \times$ inference acceleration and only requires about $1/15$ GPU memory compared with the LEDAER(T). In summary, the designed LLM-distilled medication recommendation model can get a better trade-off between performance and efficiency.








